On the group-like behaviour of the Le-Murakami-Ohtsuki invariant

We study the effect of Feynman integration and diagrammatic differential operators on the structure of group-like elements in the algebra generated by coloured vertex-oriented uni-trivalent graphs. We provide applications of our results to the study of the LMO invariant, a quantum invariant of manifolds. We also indicate further situations in which our results apply and may prove useful. The enumerative approach that we adopt has a clarity that has enabled us to perceive a number of generalizations.

==> graph3d.tex <==
\xy (0,-1.5)*{}="A"; (0,1.5)*{}="B"; (3,1.5)*{}="C";
(3,-1.5)*{}="D";(3,0)*{}="E"; (7,0)*{}="F"; "A"; "B"
**\dir{-};
"A"; "B" **\dir{-}; "B"; "C" **\dir{-}; "C"; "D" **\dir{-}; "D"; "A"
**\dir{-}; "E"; "F" **\dir{-};
"E"*{\bullet}; "F"*{\bullet}; (7,-2)*{y}; \endxy

